On the well-posedness of the Cahn-Hilliard-Biot model and its applications to tumor growth

We study the Cahn-Hilliard-Biot model with respect to its mathematical well-posedness. The system models flow through deformable porous media in which the solid material has two phases with distinct material properties. The two phases of the porous material evolve according to a generalized Ginzburg-Landau energy functional, with additional influence from both viscoelastic and fluid effects. The flow-deformation coupling in the system is governed by Biot's theory. This results in a three-way coupled system that can be viewed as an extension of the Cahn-Larche equations by adding a fluid flowing through the medium. We distinguish the cases between a spatially dependent and a state-dependent Biot-Willis function. In the latter case, we consider a regularized system. In both cases, we use a Galerkin approximation to discretize the system and derive suitable energy estimates. Moreover, we apply compactness methods to pass to the limit in the discretized system. In the case of Vegard's law and homogeneous elasticity, we show that the weak solution depends continuously on the data and is unique. Lastly, we present some numerical simulations to highlight the features of the system as a tumor growth model.

==> 5_proof_pt2.tex <==
\begin{proof}
$u_k$ is bounded in $L^\infty(H_0^1)$ and $\pt u_k$ is bounded in $L^\infty(L^2)$ and $\pt^2 u_k$ is bounded in $L^2(H^1)'$. Then we deduce 
$$L^\infty(0,T;H_0^1(\Omega)^d) \cap H^1(0,T;H_0^1(\Omega)^d) \hookrightarrow \hookrightarrow C^0([0,T];L^r(\Omega)^d),$$
 with $r$ as above, and thus we obtain the following strong convergence:
\begin{equation}
		\label{Convergence:Strong4}
			\begin{aligned}
   u_k &\to u &&\text{ strongly in } C^0([0,T];L^r(\Omega)^d), \\
     \pt u_k &\to \pt u &&\text{ strongly in } C^0([0,T];(W^{1,r'}(\Omega))').
		\end{aligned}\end{equation}
Since 
$\cup_k Y_k$ is dense in $H^1_0(\Omega)^d$, we can choose a sequence $\{
v_k\}_{k \in \N}$ with $v_k(t) \in Y_k$ for a.e. $t \in (0,T)$ and 
\begin{equation} \label{Conv:VK}\begin{aligned}v_k &\to u &&\text{ strongly in } H^1(0,T;H^1_0(\Omega)), 
\end{aligned}\end{equation}
Thus, by the convergence properties of $u_k$, see \cref{Convergence:Weak} and \cref{Convergence:Strong4}, it yields 
\begin{equation} \label{Conv:UKVK}\begin{aligned} u_k - v_k &\to 0 &&\text{ weakly* in } L^\infty(0,T;H^1_0(\Omega)^d), \\
		\pt u_k - \pt  v_k &\to 0 &&\text{ weakly* in } L^\infty(0,T;L^2(\Omega)^d), \\
u_k - v_k &\to 0 &&\text{ strongly in } C^0([0,T];L^r(\Omega)^d), \\
\pt u_k - \pt v_k &\to 0 &&\text{ strongly in } C^0([0,T];(W^{1,r'}(\Omega))').
\end{aligned}\end{equation}  Let us consider the test function $\zeta_u = u_k - v_k$
in \eqref{Sys:GalerkinVar}$_3$, which gives 
\begin{equation*}
\begin{aligned}
&(S_u,\eps(u_k-v_k))_\Omega +(\alpha p_k,\div(u_k-v_k))_\Omega \\ & =(\C_v\pt \eps(u_k),\eps(u_k-v_k))_\Omega+(\C (\phi_k)(\eps(u_k)-  \T(\phi_k)) , \eps(u_k - v_k))_\Omega 
\end{aligned}
\end{equation*}
and together with the coercivity property
\eqref{Ass:Elastic2}$_1$ it yields
\begin{equation} \label{Eq:DeriveStrongU}
\begin{aligned}&(S_u,\eps(u_k-v_k))_\Omega+(\alpha p_k,\div(u_k-v_k))_\Omega  - (\C(\phi_k)(\eps(v_k) - \T(\phi_k)), \eps(u_k - v_k))_\Omega \\
	&= (\C_v\pt \eps(u_k-v_k),\eps(u_k-v_k))_\Omega +(\C_v\pt \eps(v_k),\eps(u_k-v_k))_\Omega \\&\quad +(D_2 W(\varphi_k,\eps(u_k)) - D_2 W(\varphi_k,\eps(v_k)), \eps(u_k - v_k))_\Omega \\
& \geq C \ddt \|\eps(u_k-v_k)\|_{L^2}^2 + C \|\eps(u_k - v_k)\|_{L^2}^2  + (\C_v\pt \eps(v_k),\eps(u_k-v_k))_\Omega
\end{aligned}
\end{equation}
We note that we also have used that we can write $(\C_v \F,\mathcal{G})_\Omega=(\sqrt{\C_v} \F,\sqrt{\C_v} \mathcal{G})_\Omega$ for any $\F,\mathcal{G} \in \mathbb{R}^{n \times n}$ where $\sqrt{\C_v}$ exists according to the square-root theorem as $\C_v$ is symmetric and positive definite.
We integrate the inequality over $(0,T)$ and pass to the limit $k \to \infty$. 
The third term on the right-hand side converges to zero as $\eps(u_k-v_k)$ converges weakly to zero in $L^2(\OT)$ by \cref{Conv:UKVK} and $\pt \eps(v_k)$ converges strongly to $\pt \eps(u)$ in $L^2(\OT)$ by \cref{Conv:VK}. Similarly, the first and third terms on the left-hand side converge to zero.
The $\|\eps(u_{k,0})-\eps(v_{k,0})\|_{L^2}^2$ appears after the time integration, and it goes to zero as $\eps(u_{k,0}) \to \eps(u_0)$ in $L^2(\Omega)$ by construction of the discrete initial condition, and $\eps(v_k(0)) \to \eps(u(0))$  by the strong convergence of $v_k$ in $C([0,T];H_0^1(\Omega))$, see \cref{Conv:VK}. It remains to treat the second term on the left-hand side of the inequality. First, we integrate by parts and exploit the homogeneous Dirichlet boundary condition of $u_k-v_k$ to get
$$(\alpha(\phi_k) p_k,\div(u_k-v_k))_\OT =-(\alpha' p_k,u_k-v_k)_\OT - (\alpha \nabla p_k,u_k-v_k)_\OT.
$$
Here, we use the strong convergence of $u_k-v_k$ to zero in $L^2(\OT)$ together with the weak convergence of $p_k$ and $\nabla p_k$ in $L^2(\OT)$. We note that in the case of a state dependent Biot--Willis function $\phi_k \mapsto \alpha(\phi_k)$, an additional term $\nabla \phi_k$ would appear after integration by parts and we would require strong convergence of this term to pass to the limit.
Collecting all the derived convergences, we see from \cref{Eq:DeriveStrongU} that
\begin{align*}
\|\eps(u_k - v_k)\|_{L^2(\Omega_T)}^2 \to 0 \quad \text{ as } k \to \infty.
\end{align*}
By Korn's inequality this shows that $u_k-v_k$ converges strongly to zero in the space $L^2(0,T;H^1_0(\Omega))$ and hence 
\begin{equation} \label{Eq:StrongU2} u_k \to u \quad \text{ strongly in }  L^2(0,T;H^1_0(\Omega)).
\end{equation} %


Next, we consider the discretized pressure equation and, having already derived the strong convergence of $u_k$, we are able to conclude a strong convergence result for $p_k$. As $\cup_k Z_k$ is dense in $H^1(\Omega)$, we can choose a sequence $\{q_k\}$ with $q_k(t) \in Z_k$ for a.e. $t \in (0,T)$ and $q_k \to p$ strongly in $L^2(0,T;H^1(\Omega))$. Then, it also yields $p_k-q_k \to 0$ weakly in $L^2(0,T;H^1(\Omega))$. We consider the test function $\xi_p=p_k-q_k$ in \eqref{Sys:GalerkinVar}$_5$, which gives after integration
\begin{equation} \label{Eq:PkQk} \begin{aligned} \|p_k-q_k\|^2_{L^2(\OT)} &= (q_k,p_k-q_k)_\OT  -(\alpha M(\phi_k) \div u_k, p_k-q_k)_\OT 
	\\&\quad +(M(\phi_k) \theta_k,p_k-q_k)_\OT .\end{aligned}\end{equation}
The terms on the right-hand side all converge to zero as $k \to \infty$.
In fact, $q_k$ strongly converges in $L^2(\OT)$ and $p_k-q_k$ weakly converges to $0$ in $L^2(\OT)$. Furthermore, we have just derived that $\div u_k$ strongly converges in $L^2(\OT)$ and together with the boundedness of $M$ and the strong convergence of $\phi_k$, we conclude that $M(\phi_k) \div u_k$ converges strongly in $L^2(\OT)$. 
 The third term remains to be treated. %
 We have
\begin{equation} \label{Eq:PuzzlePiece} \begin{aligned} &\left( M(\phi_k) \theta_k,   p_k-q_k \right)_\OT\\
&=\left( M(\phi_k)\theta_k-M(\phi)\theta,  p_k-q_k  \right)_\OT+ \left( M(\phi)\theta,  p_k-q_k \right)_\OT \\
&\leq \|M(\phi_k)\theta_k-M(\phi)\theta\|_{L^2(H^1)'} \|p_k-q_k\|_{L^2(H^1)}+ \left( M(\phi)\theta,  p_k-q_k \right)_\OT.
\end{aligned} \end{equation}
We observe that the second term converges to zero as $M(\phi) \theta \in L^2(\OT)$ and $p_k-q_k$ converges weakly to zero in $L^2(\OT)$. From the weak convergence of $p_k-q_k$ in $L^2(0,T;H^1(\Omega))$ we are also able to conclude  that $p_k-q_k$ is bounded in said space. We prove that the first norm in the first term on the right-hand side goes to zero. %
We first note that
$$M(\phi_k) \theta_k - M(\phi) \theta = M(\phi_k) (\theta_k-\theta) - (M(\phi_k)-M(\phi)) \theta,$$
and here the second term converges to zero in $L^2(\OT)$ by the dominated convergence theorem as $M(\phi_k)\theta \to M(\phi) \theta$ a.e. in $\OT$ and the sequence is uniformly bounded in $L^2(\Omega)$. The first term goes to zero as
$$\begin{aligned} \|M(\phi_k) (\theta_k-\theta)\|_{L^2(H^1)'} &=\sup_{\|\xi\|_{L^2(H^1)} \leq 1} |(\theta_k-\theta,M(\phi_k)\xi)_\OT |  \\ 
	&\leq \sup_{\|\xi\|_{L^2(H^1)}\leq 1} \|\theta_k-\theta\|_{L^2(W^{1,4/3})'} \|M(\phi_k) \xi\|_{L^2(W^{1,4/3})} 
	\end{aligned}$$
and we have for any $\xi \in L^2(0,T;H^1(\Omega))$
$$\begin{aligned}
	\|M(\phi_k) \xi\|_{L^2(L^{4/3})}  &\leq M_\infty \|\xi\|_{L^2(L^{4/3})} \leq C  \|\xi\|_{L^2(L^2)}, \\
	\|M(\phi_k) \nabla \xi\|_{L^2(L^{4/3})}  &\leq M_\infty \|\nabla \xi\|_{L^2(L^{4/3})} \leq C  \|\nabla \xi\|_{L^2(L^2)}, \\
	\|M'(\phi_k) \nabla \phi_k \xi\|_{L^2(L^{4/3})}  &\leq M'_\infty \|\nabla \phi_k\|_{L^\infty(L^2)} \|\xi\|_{L^2(L^{4})} \leq C  \|\xi\|_{L^2(H^1)}, 
\end{aligned}$$
where we used H\"older's inequality with $\frac{1}{2}+\frac{1}{4}=\frac{3}{4}$ and the $k$-uniform bound of $\nabla \phi_k$ in $L^\infty(0,T;L^2(\Omega))$. Thus, $M(\phi_k) (\theta_k-\theta)$ converges to zero in $L^2(0,T;(H^1(\Omega))')$.  Hence, the term in \eqref{Eq:PuzzlePiece} and likewise in \eqref{Eq:PkQk} goes to zero.  We conclude
$p_k-q_k \to 0$ in $L^2(\OT)$ and 
$$p_k \to p \quad \text{ strongly in} L^2(\OT).$$

Again, we consider the discretized pressure equation and, having already derived the strong convergence of $u_k$ and $p_k$, we are able to conclude a strong convergence result for $\theta_k$. As $\cup_k Z_k$ is dense in $L^2(\Omega)$, we can choose a sequence $\{\Theta_k\}$ with $\Theta_k(t) \in Z_k$ for a.e. $t \in (0,T)$ and $\Theta_k \to \theta$ strongly in $L^2(\OT)$. Then, it also yields $\theta_k-\Theta_k \to 0$ weakly in $L^2(\OT)$. We consider the test function $\xi_p=\theta_k-\Theta_k$ in \eqref{Sys:GalerkinVar}$_5$, which gives after integration
\begin{equation} \label{Eq:PkQk2} \begin{aligned} M_0^2 \| \theta_k-\Theta_k\|^2_{L^2(\OT)}  &\leq \|M(\phi_k)(\theta_k-\Theta_k)\|^2_{L^2(\OT)} \\ &= (M(\phi_k) \Theta_k ,\theta_k-\Theta_k)_\OT + (p_k,\theta_k-\Theta_k)_\OT  \\ &\quad  +(\alpha M(\phi_k) \div u_k, \theta_k-\Theta_k)_\OT.
\end{aligned} \end{equation}
The right-hand side is converging to zero as $k \to \infty$ by the weak convergence of $\theta_k-\Theta_k$ and the strong convergences of $\Theta_k$, $p_k$, $\div u_k$. We conclude
$$\theta_k \to \theta \quad \text{ strongly in} L^2(\OT).$$



		
		
		\noindent\textbf{Step 4 (Energy inequality and initial conditions).} We note that the energy inequality \cref{Est:Final} holds in a continuous setting in the sense that we may replace $\phi_k$ by $\phi$ and so on. This is achieved by taking the limit inferior as $k \to \infty$ and using that norm are weakly/weakly* lower semicontinuous. Moreover, we apply the Fatou lemma on the non-negative continuous function $\Psi$ to achieve
		$$\int_\Omega \Psi(\phi(x)) \dx \leq \liminf_{k \to \infty}\int_\Omega \Psi(\phi_k(x)) \dx.$$
		Thus, the quintuple $(\phi,\mu,u,\theta,p)$ satisfies \cref{Est:FinalCont} as stated in \cref{Theorem}.
  
		Regarding the initial conditions, we note that it holds $\phi_k(0) \to \phi(0)$ in $L^r(\Omega)$ as $k \to \infty$ according to the strong convergence \cref{Convergence:Strong} by setting $t=0$. However, it holds $\phi_k(0)=\phi_{k,0} \to \phi_0$ in $H^1(\Omega)$ by the definition of $\phi_{k,0}=\Pi_{Z_k} \phi_0$ and the properties of the orthogonal projection. Thus, we obtain $\phi(0)=\phi_0$ in $L^r(\Omega)$ by the uniqueness of limits. Moreover, we make use of the embedding, see \cite[Lemma II.5.9]{boyer2012mathematical}
		$$C([0,T];L^r(\Omega)) \cap L^\infty(0,T;H^1(\Omega)) \hookrightarrow C_w([0,T];H^1(\Omega)),$$
		to infer that $\phi$ is weakly continuous with values in $H^1(\Omega)$ and thus, the initial condition $\phi_0$ is satisfied in the sense
		$$\langle w,\phi(t) \rangle_{H^1} \to \langle w,\phi_0 \rangle_{H^1} \quad \forall w \in (H^1(\Omega))'.$$ In the same manner, we obtain $u(0)=u_0$ in $L^r(\Omega)$ and $\theta(0)=\theta_0$ in $L^2(\Omega)$.
  \smallskip
		
		\noindent\textbf{Step 5 (Limit process).} In this step, we pass to the limit $k \to \infty$ in the $k$-th Galerkin system using the convergences that we have derived in \cref{Convergence:Weak}--\cref{Convergence:Strong2}. First, we multiply each of the Galerkin equations \cref{Sys:GalerkinVar} by an arbitrary function $\eta \in C_0^\infty(0,T)$ and integrate over $(0,T)$, giving
		\begin{equation} \label{Sys:GalerkinVarInt} \begin{aligned}
				\langle \pt \phi_k,\eta z\rangle_{L^2(H^1)} + (m(\phi_k)\nabla \mu_k,\eta\nabla z)_\OT&=  (S_\phi(\phi_k),\eta z)_\OT, \\
				- (\mu_k,\eta z)_\OT+\gamma  (\nabla\phi_k,\eta \nabla z)_\OT + (\Psi'(\phi_k),\eta z)_\OT &= -(\delta_{\phi_k} \E_\theta^k + \delta_{\phi_k} \E_u^k,\eta z)_\OT,    \\
				(\C_v\pt \eps(u_k),\eta \eps(y))_\OT +\big(\mathbb{C}(\varphi_k)\left({ \varepsilon}( u_k)-\mathcal{T}(\varphi_k)\right),\eta \nabla y\big)_\OT &=  (\alpha p_k,\eta \div y)_\OT, \\
				\langle\pt \theta_k,\eta z\rangle_{L^2(H^1)} + (\kappa(\phi_k)\nabla p_k,\eta \nabla z)_\OT  &= (S_\theta(\phi_k),\eta z)_\OT, \\
				(M(\phi_k)(\theta_k-\alpha \div u_k), \eta z)_\OT   &= (p_k,\eta z)_\OT,   
		\end{aligned}\end{equation}
		for any $z \in Z_k$, $y \in Y_k$ and $\eta \in C_0^\infty(0,T)$.
		
		Taking the limit $k \to \infty$ in the linear terms such as $(p_k,\eta z)_{\OT}$ follows directly due to the weak convergences \cref{Convergence:Weak}. Therefore, we only study the nonlinearities. We notice that the nonlinear functions terms depending on $\phi_k$ (such as $\kappa(\phi_k)$) are bounded. The convergence of these terms can be treated using the strong convergence of $\phi_k$, see \cref{Convergence:Strong}, and the Lebesgue dominated convergence theorem. By the weak-strong convergence lemma, we can take the limit in all the product-structured terms such as $(m(\phi_k)\nabla \mu_k,\eta \nabla z)_{\OT}$. 
  
  Due to the strong convergence $u_k \to u$ in $L^2(0,T;H_0^1(\Omega))$ and the growth estimates of $W$ and its derivatives, see \cref{Ass:Elastic2}, we can pass to the limit in $\delta_{\phi_k} \E_u^k$. Further, we use the strong convergence of $\theta_k$ and $u_k$ to pass the limit in the quadratic nonlinearities in $\delta_{\phi_k} \E_\theta^k$.
  
  Then we use that $\cup_k Z_k$ is dense in $H^1(\Omega)$ and $\cup_{k} Y_k$ is dense in $H_0^1(\Omega)^d$. Together with the fundamental lemma of calculus of variations, it yields that $(\phi,\mu,u,\theta,p)$ is a weak solution to the Cahn--Hilliard--Biot system in the sense of \cref{Definition}. \end{proof}

  We have proved the existence of a weak solution. Next, we prove the uniqueness and continuous dependence on the data of the said solution in the case of stricter assumptions, as stated in \cref{Thm:Uniqueness}.

  \begin{proof}[Proof of \cref{Thm:Uniqueness}]
Now, we are in the setting that $m(\phi)=m$, $\C(\phi)=\C$, $\kappa(\phi)=\kappa$, $\alpha(\phi)=\alpha$, $M(\phi)=M$ are constant and $\T(\phi)$ is affine linear i.e. $\T(\phi)=\T_1+\T_2\phi$. In particular, this implies $$D_\phi W(\phi,\eps(u))=-\C(\eps(u)-\T_1-\T_2\phi):\T_2.$$
Moreover, due to $\alpha'=M'=0$, we have $\delta_\phi \E_\theta=0$.
In this case, we can easily prove that it holds $\phi \in L^2(0,T;H^2(\Omega))$ by solving the equation of the chemical potential $\mu$ for $\Delta \phi$.
Therefore, the inverse Neumann--Laplacian is well-defined when applying it to $\phi$.

		We consider two weak solutions $(\phi_1,\mu_1,u_1,\theta_1,p_1)$ and $(\phi_2,\mu_2,u_2,\theta_2,p_2)$, and we denote their difference by $\phi=\phi_1-\phi_2$ and in the same way for the other variables. Subtracting their weak forms, we obtain
			\begin{equation} \label{Eq:UniqueTest1}\begin{aligned}
			\langle\pt \phi,\zeta_\phi\rangle_{H^1} + m(\nabla \mu,\nabla \zeta_\phi)_\Omega&=(S_\phi(\phi_1)-S_\phi(\phi_2),\zeta_\phi)_\Omega, \\
			- (\mu,\zeta_\mu)_\Omega+\gamma  (\nabla\phi,\nabla \zeta_\mu)_\Omega + (\Psi'(\phi_1)\!-\!\Psi'(\phi_2),\zeta_\mu)_\Omega &= -(\C(\eps(u)\!-\!\T_2\phi),\T_2\zeta_\mu)_\Omega,  \\
			(\C_v \eps(\pt u),\eps(\zeta_u))_\Omega+\big(\C\big({ \varepsilon}( u)-\T_2\varphi\big),\eps(\zeta_u)\big)_\Omega &= \alpha(p,\div \zeta_u)_\Omega,  \\
			\langle\pt \theta,\zeta_\theta\rangle_{H^1} + \kappa(\nabla p,\nabla\zeta_\theta)_\Omega  &= (S_\theta(\phi_1)-S_\theta(\phi_2),\zeta_\theta)_\Omega, \\
			(p,\zeta_p)_\Omega   &= M(\theta-\alpha \div u,\zeta_p)_\Omega,  
		\end{aligned} \end{equation}
		for any $\zeta_\phi, \zeta_\mu,\zeta_\theta,\zeta_p \in H^1(\Omega)$, $\zeta_u \in H^1_0(\Omega)$. 
		We have $p=M(\theta-\alpha \div u)$ in $L^2(\OT)$. Moreover, as the right-hand side is in $L^2(0,T;(H^1(\Omega))')$, we obtain $\pt p = M \pt \theta- \alpha \div \pt u$ in $L^2(0,T;(H^1(\Omega))')$. From here, we see that
		\begin{equation} \label{Eq:UniqueTest2} \langle\pt p,\zeta_\theta\rangle_{H^1} + M\kappa(\nabla p,\nabla\zeta_\theta)_\Omega  = (S_\theta(\phi_1)-S_\theta(\phi_2),\zeta_\theta)_\Omega - \alpha (\div \pt u,\zeta_\theta)_\Omega,
			\end{equation} 
		for any $\zeta_\theta \in H^1(\Omega)$ and the initial condition $p(0)=p_0:=M \theta_0 - \alpha \div u_0 \in L^2(\Omega)$.
				\medskip
		
		\noindent\textbf{First testing.} Taking the test functions $\zeta_\phi=(-\Delta)^{-1} \phi$ in \eqref{Eq:UniqueTest1}$_1$ and $\zeta_\mu=m\phi$ in \eqref{Eq:UniqueTest1}$_2$, it yields
		\begin{equation*} 
			\begin{aligned}
				\langle \p_t \phi,(-\Delta)^{-1} \phi\rangle_{H^1} + m (\nabla \mu,\nabla (-\Delta)^{-1} \phi)_\Omega &= (S_\phi(\phi_1)-S_\phi(\phi_2),(-\Delta)^{-1}\phi)_\Omega, \\
				-m(\mu,\phi)_\Omega+ m\gamma (\nabla \phi,\nabla \phi)_\Omega &= - m(\Psi'(\phi_1)-\Psi'(\phi_2),\phi)_\Omega \\ &\quad\, -m(\C(\eps(u)\!-\!\T_2\phi),\T_2\varphi)_\Omega  
			\end{aligned}
		\end{equation*} 
		Exploiting the property $(\nabla \mu, \nabla (-\Delta)^{-1} \phi)_\Omega = (\mu,\phi)_\Omega$ of the Neumann--Laplace operator,  after adding the equations and canceling, it yields
		\begin{equation} \label{Eq:UniqueDifference}
			\begin{aligned}
				&\langle \p_t \phi, (-\Delta)^{-1} \phi\rangle_{H^1} + m \gamma \|\nabla \phi\|_{L^2}^2 + m(\Psi'(\phi_1)-\Psi'(\phi_2),\phi)_\Omega \\
				&=(S_\phi(\phi_1)-S_\phi(\phi_2),(-\Delta)^{-1} \phi)_\Omega - m(\C(\eps(u)\!-\!\T_2\phi),\T_2\varphi)_\Omega. 
			\end{aligned}
		\end{equation}
  The graph norm $\|\nabla (-\Delta)^{-1} \cdot\|_{L^2}$ is equivalent to the usual norm of $(H^1(\Omega))'$. Thus, we set $\|\cdot\|_{(H^1)'}=\|\nabla (-\Delta)^{-1} \cdot\|_{L^2}$. First, we note that we may rewrite the first term on the left-hand side of \cref{Eq:UniqueDifference} as %
		\begin{equation}  
			\begin{aligned} 
				\langle \p_t \phi, (-\Delta)^{-1} \phi\rangle_{H^1} &= \langle -\Delta (-\Delta)^{-1} \p_t \phi, (-\Delta)^{-1} \phi\rangle_{H^1}  \\&= \langle\p_t \nabla (-\Delta)^{-1} \phi, \nabla (-\Delta)^{-1} \phi\rangle_{H^1} \\
				&= \frac12 \ddt \|\phi\|_{(H^1)'}^2.
			\end{aligned} \label{Eq:UniqueChain} 
		\end{equation}
		Using the semiconvexity of $\Psi$, see \cref{Ass:PsiNew}, it yields
		$$m(\Psi'(\phi_1)-\Psi'(\phi_2),\phi)_\Omega \geq - C_* m\|\phi\|_{L^2}^2,
		$$
		and consequently, we obtain by the Young inequality 
	\begin{equation} \label{Eq:L2EstimateInvLap}\begin{aligned}m(\Psi'(\phi_2)-\Psi'(\phi_1),\phi)_\Omega &\leq C_*m \|\phi\|_{L^2}^2 \\ &= C_*m (\nabla (-\Delta)^{-1} \phi,\nabla \phi)_\Omega \\ &\leq \frac{m\gamma}{4} \|\nabla \phi\|^2_{L^2} + \frac{C_*^2m}{\gamma} \|\nabla (-\Delta)^{-1} \phi\|_{L^2}^2.\end{aligned}\end{equation}
Here, we have seen that we can estimate any $L^2(\Omega)$-norm of $\phi$ using the Laplacian and inverse Laplacian operators. This property is also used in the next step.
		Using the Lipschitz continuity of $S_\phi$, see \cref{Ass:FunNew}, the right-hand side of \cref{Eq:UniqueDifference} can be treated  as follows:
		$$\begin{aligned}
			&(S_\phi(\phi_1)-S_\phi(\phi_2),(-\Delta)^{-1} \phi)_\Omega - m(\C(\eps(u)\!-\!\T_2\phi),\T_2\varphi)_\Omega  \\
			&\leq C \|\phi\|_{L^2} \|(-\Delta)^{-1} \phi\|_{L^2} + C \|\eps(u)\|_{L^2} \|\phi\|_{L^2} + C\|\phi\|_{L^2}^2   \\
			&\leq \frac{m\gamma}{4} \|\nabla \phi\|_{L^2}^2  + C\|\phi\|_{(H^1)'}^2 +  \frac{C_\C}{4} \|\eps(u)\|_{L^2}^2.
		\end{aligned}$$
		Therefore, applying this estimate and \cref{Eq:UniqueChain} to \cref{Eq:UniqueDifference}, it yields
		\begin{equation}  \label{Est:UniqueFinal1}
			\begin{aligned}
				\frac12 \ddt \|\phi\|_{(H^1)'}^2 + \frac{m \gamma}{2} \|\nabla \phi\|_{L^2}^2 \leq C\|\phi\|_{(H^1)'}^2 +\frac{C_\C}{4} \|\eps(u)\|_{L^2}^2.
			\end{aligned}
		\end{equation} \smallskip
	
\noindent\textbf{Second testing.}		Next, we consider the test functions $\zeta_u=\pt u$ in \eqref{Eq:UniqueTest1}$_3$, $z_p=\theta$ in  \eqref{Eq:UniqueTest1}$_5$, $z_\theta=p$ in \eqref{Eq:UniqueTest2} to obtain
		$$\begin{aligned} C_\C \|\pt \eps(u)\|_{L^2}^2 + \frac{1}{2} \ddt \|\C^{1/2}\eps(u)\|_{L^2}^2  &= \big(\C\T_2\varphi,\eps(\pt u)\big)_\Omega+\alpha  (p,\div \pt u)_\Omega,  \\
			  M \|\theta\|_{L^2}^2  &= (p,\theta)_\Omega + \alpha M (\div u,\theta)_\Omega, \\
			\frac12 \ddt \|p\|_{L^2}^2 + M \kappa \|\nabla p\|_{L^2}^2 &= (S_\theta(\phi_1)-S_\theta(\phi_2),p) - \alpha (\div \pt u,p)_\Omega,
		 %
		\end{aligned}$$
	where we have used that $\C$ (and $\C^{1/2}$) is positive definite and thus self-adjoint.
		Adding the tested equations gives
		$$\begin{aligned}
			&C_\C \|\pt\eps(u)\|_{L^2}^2+C\ddt \|\eps(u)\|_{L^2}^2+ M \|\theta\|_{L^2}^2+\frac12 \ddt \|p\|_{L^2}^2+ M\kappa \|\nabla p\|_{L^2}^2 \\
   &= (\C(\T_2\phi),\eps(\pt u))_\Omega  +(p,\theta)_\Omega + \alpha M (\div u,\theta)_\Omega+(S_\theta(\phi_1)-S_\theta(\phi_2),p)_\Omega 
		\end{aligned}$$
  We apply the H\"older inequality on the terms on the right-hand side of this equality and with the boundedness of $S_\theta$, see \cref{Ass:Fun}, we obtain
  		\begin{equation}\label{Est:Unique2}\begin{aligned}
			&C_\C \|\pt\eps(u)\|_{L^2}^2+C \ddt \|\eps(u)\|_{L^2}^2+M \|\theta\|_{L^2}^2+\frac12 \ddt \|p\|_{L^2}^2+ M\kappa \|\nabla p\|_{L^2}^2 \\
			&\leq  C \|\phi\|_{L^2} \|\pt \eps(u)\|_{L^2}+C \|p\|_{L^2} \|\theta\|_{L^2} + C \|\div u\|_{L^2} \|\theta\|_{L^2} + C \|\phi\|_{L^2} \|p\|_{L^2}
		\end{aligned}\end{equation}
  We apply the Young inequality on the right-hand side of the inequality. In particular, we have for the terms where $\phi$ appears
  $$\begin{aligned}&C \|\phi\|_{L^2} \|\eps(u)\|_{L^2}+C\|\phi\|_{L^2} \|p\|_{L^2} \\ &\leq 
  	C\|\phi\|_{L^2}^2 + \frac{C_\C}{2} \|\pt \eps(u)\|_{L^2}^2 + C \|p\|_{L^2}^2  \\
  	&\leq C \|\phi\|_{(H^1)'}^2 + \frac{m\gamma}{4} \|\nabla \phi\|_{L^2}^2+ \frac{C_\C}{2} \|\pt \eps(u)\|_{L^2}^2 + C \|p\|_{L^2}^2 ,
  \end{aligned}$$
  where we applied \cref{Eq:L2EstimateInvLap} to estimate $\phi$ in the $L^2(\Omega)$-norm in the last step.
  Inserting this estimate into \cref{Est:Unique2}, we obtain
\begin{equation}  \label{Est:UniqueFinal2}	\begin{aligned}
		&\frac{C_\C}{2} \|\pt\eps(u)\|_{L^2}^2+C \ddt \|\eps(u)\|_{L^2}^2+\frac{M}{2} \|\theta\|_{L^2}^2+\frac12 \ddt \|p\|_{L^2}^2+ M\kappa \|\nabla p\|_{L^2}^2 \\
		&\leq C \|\phi\|_{(H^1)'}^2 + \frac{m\gamma}{4} \|\nabla \phi\|_{L^2}^2+  C \|p\|_{L^2}^2+C\|\eps(u)\|_{L^2}^2.
    \end{aligned}\end{equation}
\smallskip

    



		
		\noindent\textbf{Together.}
  We add \cref{Est:UniqueFinal1} to   \cref{Est:UniqueFinal2}, which gives
  \begin{equation*}  \begin{aligned}
			&\frac12 \ddt \|\phi\|_{(H^1)'}^2 +\frac{m \gamma}{4} \|\nabla \phi\|_{L^2}^2+\frac{C_\C}{2} \|\pt \eps(u)\|_{L^2}^2 +C \ddt \|\eps(u)\|_{L^2}^2 + \frac{M}{2} \|\theta\|_{L^2}^2  \\ &\quad  +\frac{1}{2} \ddt \|p\|_{L^2}^2 + M\kappa \|\nabla p\|_{L^2}^2 \\
  		&\lesssim   \|\phi\|_{(H^1)'}^2 + \|p\|_{L^2}^2 + \|\eps(u)\|_{L^2}^2.
    \end{aligned}\end{equation*}
		We integrate and apply the Gronwall inequality, which gives, after taking the essential supremum of $t\in(0,T)$,
		\begin{equation*} %
			\begin{aligned}
				& \|\phi\|_{L^\infty(H^1)' \cap L^2(L^2)}^2+ \|\pt u\|_{L^2(H_0^1) }^2+\| u\|_{L^\infty(H_0^1) }^2 + \|\theta\|_{L^2(L^2)}^2 +   \|p\|_{L^\infty(L^2) \cap L^2(H^1)}^2\\ &\lesssim  \|\phi_{0,1}-\phi_{0,2} \|_{(H^1)'}^2 +\|u_{0,1}-u_{0,2} \|_{H^1}^2 + \|p_{0,1}-p_{0,2}\|_{L^2}^2.
			\end{aligned}
		\end{equation*}
	As noted before, we may use the representation of the initial pressure to estimate the last term on the right-hand side as follows:
	$$\|p_{0,1}-p_{0,2}\|_{L^2}^2 \leq C \|\theta_{0,1}-\theta_{0,2}\|_{L^2}^2 + C \|u_{0,1}-u_{0,2}\|_{H^1}^2.$$
    Moreover, from \cref{Eq:UniqueTest1}$_2$ we have that
    $$\|\mu\|_{L^2(H^1)'}^2 \lesssim \|\phi\|_{L^2(H^1)} + \|\eps(u)\|_{L^2(L^2)}^2.$$
  This completes the continuous dependence on the data as stated in \cref{ContDep}.
Moreover, in the case of $\phi_{0,1}=\phi_{0,2}$, $u_{0,1}=u_{0,2}$ and $\theta_{0,1}=\theta_{0,2}$, the weak solutions coincide. 
	\end{proof}
